HPFF: Hierarchical Locally Supervised Learning with Patch Feature Fusion

Traditional deep learning relies on end-to-end backpropagation for training, but it suffers from drawbacks such as high memory consumption and not aligning with biological neural networks. Recent advancements have introduced locally supervised learning, which divides networks into modules with isolated gradients and trains them locally. However, this approach can lead to performance lag due to limited interaction between these modules, and the design of auxiliary networks occupies a certain amount of GPU memory. To overcome these limitations, we propose a novel model called HPFF that performs hierarchical locally supervised learning and patch-level feature computation on the auxiliary networks. Hierarchical Locally Supervised Learning (HiLo) enables the network to learn features at different granularity levels along their respective local paths. Specifically, the network is divided into two-level local modules: independent local modules and cascade local modules. The cascade local modules combine two adjacent independent local modules, incorporating both updates within the modules themselves and information exchange between adjacent modules. Patch Feature Fusion (PFF) reduces GPU memory usage by splitting the input features of the auxiliary networks into patches for computation. By averaging these patch-level features, it enhances the network's ability to focus more on those patterns that are prevalent across multiple patches. Furthermore, our method exhibits strong generalization capabilities and can be seamlessly integrated with existing techniques. We conduct experiments on CIFAR-10, STL-10, SVHN, and ImageNet datasets, and the results demonstrate that our proposed HPFF significantly outperforms previous approaches, consistently achieving state-of-the-art performance across different datasets. Our code is available at: https://github.com/Zeudfish/HPFF.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}

\makeatletter{\renewcommand*{\@makefnmark}{}
\footnotetext{$^*$Equal Contribution. \\
\Letter  Corresponding Author: Chengyang Si (chenyang.si.mail@gmail.com).}}

Traditional deep learning relies on end-to-end backpropagation for training, but it suffers from drawbacks such as high memory consumption and not aligning with biological neural networks. Recent advancements have introduced locally supervised learning, which divides networks into modules with isolated gradients and trains them locally. However, this approach can lead to performance lag due to limited interaction between these modules, and the design of auxiliary networks occupies a certain amount of GPU memory. To overcome these limitations, we propose a novel model called HPFF that performs hierarchical locally supervised learning and patch-level feature computation on the auxiliary networks. Hierarchical Locally Supervised Learning (HiLo) enables the network to learn features at different granularity levels along their respective local paths. Specifically, the network is divided into two-level local modules: independent local modules and cascade local modules. The cascade local modules combine two adjacent independent local modules, incorporating both updates within the modules themselves and information exchange between adjacent modules. Patch Feature Fusion (PFF) reduces GPU memory usage by splitting the input features of the auxiliary networks into patches for computation. By averaging these patch-level features, it enhances the network's ability to focus more on those patterns that are prevalent across multiple patches. Furthermore, our method exhibits strong generalization capabilities and can be seamlessly integrated with existing techniques. We conduct experiments on CIFAR-10, STL-10, SVHN, and ImageNet datasets, and the results demonstrate that our proposed HPFF significantly outperforms previous approaches, consistently achieving state-of-the-art performance across different datasets. Our code is available at: \url{https://github.com/Zeudfish/HPFF}.

 \keywords{Local Learning \and Image Classification \and Hierarchical Locally Supervised Learning \and Patch Feature Fusion}
 
\end{abstract}

==> sec/1_intro.tex <==
% \section{Introduction}
% \label{sec:intro}
% Deep learning frameworks, such as those detailed in \cite{huang2017densely, krizhevsky2012imagenet, lecun2015deep, ren2022scaling}, predominantly employ end-to-end backpropagation \cite{rumelhart1986learning} for their learning processes. Despite its notable success in the realm of deep learning, this technique is at odds with our understanding of human learning, which typically involves local synaptic transmissions \cite{hebb1949}. In essence, the principles of end-to-end backpropagation run counter to our neurobiological characteristics.

% The end-to-end backpropagation process \cite{rumelhart1985learning} necessitates that the updates to signals in earlier neurons are postponed until the subsequent neurons have been updated. This method contradicts our understanding of human neural characteristics \cite{crick1989recent, kruberg2021biological}. Furthermore, a network training perspective reveals that the update of hidden layers \cite{rumelhart1985learning} must be deferred until the supervisory signals of the output layer \cite{siddiqui2022blockwise} are complete. This requirement leads to the storage of extensive weight data, consequently consuming substantial memory resources.

% In response to these challenges, a novel learning methodology, termed local learning, has emerged \cite{belilovsky2019greedy,mostafa2018deep,bengio2006greedy,nokland2019training,illing2021local,wang2021revisiting}. This approach segments end-to-end backpropagation independently, dividing the network into various subnetworks. Each of these subnetworks undergoes independent backpropagation for supervision. Unlike traditional end-to-end methods, lower-layer networks with this approach do not need to wait for the global loss signal from the upper layer. Each block can independently generate supervisory signals for its local module, leading to a significant speed-up in weight updates. This method enables each sub-block to concentrate on the current block, thereby learning more local features. Furthermore, while end-to-end backpropagation requires weight storage from a previous update to await the upper-layer supervisory signal needed for the current update, local learning efficiently addresses this issue and substantially reduces memory consumption. From a biological perspective, the local learning method aligns more closely with human neural characteristics.

% However, as pointed out by \cite{bengio2006greedy, belilovsky2019greedy}, lower-layer blocks might overemphasize local features. While this can enhance local performance, over-learning lower-level local information can trap the network in local optima, thereby compromising the global performance of local learning in comparison to traditional backpropagation.

% Subsequent studies \cite{xiong2020loco, wang2021revisiting, siddiqui2023blockwise} have endeavored to tackle this issue. InfoPro \cite{wang2021revisiting} refined the loss function to guarantee that the gradient-isolated network module maintains features beneficial to the overall network during the learning process. However, these methods cannot solve the issue of insufficient interaction between modules, resulting in disappointing performance when the network is divided into a large number of modules. The performance is particularly unsatisfactory when applied to large datasets {\cite{deng2009imagenet}}.


% \begin{figure*}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=\linewidth]{sec/6(2)_20231019180853_00.png}

%    \caption{The HiLo overall architecture. 
%    Where (a) is the structure diagram of E2E training, (b) is the structure diagram of other supervised local learning, (c) is the structure diagram of HiLo. We divide the backbone into K blocks in the figure.}
%    \label{Figure 1}
% \end{figure*}
% In this paper, we propose a solution to this problem, which we refer to as Hierarchical Locally Supervised Learning (HiLo). HiLo comprises two forward paths with identical structures but different granularities. The weights of the same module in the different forward paths are shared. Both forward paths adopt a method based on supervised local learning, where the networks in the two forward paths produce different losses through different auxiliary networks. After applying weights, these two losses are summed up to update the weights of the two gradient-isolated network modules simultaneously. The two losses at different granularities can learn different characteristics, thereby compensating for each other's shortcomings. Our overall contributions are as follows:

% \begin{itemize}
%     \item We have proposed a network structure for the first time in the field of supervised local learning that can truly solve the problem of information interaction between layers.
%     \item We have proposed a universal method in the field of supervised local learning, which can be plug-and-play in any supervised local learning methods.
%     \item Our proposed HiLo greatly enhances the performance of supervised local learning methods, achieving state-of-the-art results while significantly saving GPU memory compared to E2E method.
% \end{itemize}




% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.2\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio, height=1\textwidth]{sec/6(2)_20231017232948_00.png}
%     \caption{Feature Map of Forward1}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hspace{0.02\linewidth}
%   \begin{subfigure}{0.2\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio, height=1\textwidth]{sec/6(2)_20231017232948_01.png}
%     \caption{Feature Map of Forward2}
%     \label{fig:short-b}
%   \end{subfigure}
%   \hspace{0.02\linewidth}
%   \begin{subfigure}{0.2\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio, height=1\textwidth]{sec/6(2)_20231017232948_02.png}
%     \caption{Feature Map of HiLo}
%     \label{fig:short-c}
%   \end{subfigure}
%   \begin{subfigure}{0.2\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth,keepaspectratio, height=1\textwidth]{sec/6(2)_20231017232948_03.png}
%     \label{fig:short-a}
%   \end{subfigure}
%   \caption{Visualization of channel feature maps. 
%   Visualization of intermediate layer features for forward 1 and forward 2}
%   \label{fig:short}
% \end{figure*}
% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=1\linewidth]{sec/img_v2_cf334c80-f00f-43e0-8640-d1b49d50135g.jpg}

%    \caption{Visualization of dual channel feature maps. 
%    Visualization of HiLo middle layer features}
%    \label{fig:onecol}
% \end{figure}

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.5\linewidth}
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=1\linewidth]{sec/img_v2_27af5d9b-da10-42b1-8c61-8e71e2a7559g.jpg}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.5\linewidth}
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=1\linewidth]{sec/img_v2_5dfaded8-61c1-4fac-aa26-86f1391e45eg.jpg}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

\section{Introduction}
\label{sec:intro}
Deep learning frameworks, such as those detailed in \cite{huang2017densely, krizhevsky2012imagenet, lecun2015deep, ren2022scaling}, predominantly employ end-to-end backpropagation \cite{rumelhart1986learning} for their learning processes. 
Despite its notable success in the realm of deep learning, the technique are trained end-to-end with the backpropagation algorithm (BP) , which faces several limitations.
On one hand, Backpropagation (BP) presents biological implausibility \cite{crick1989recent}\cite{shen2022backpropagation} , as it relies on a global objective optimized by backpropagating error signals across layers.
On the other hand, The end-to-end backpropagation process introduces the update locking problem \cite{jaderberg2017decoupled}, where hidden layer parameters cannot be updated until both forward and backward computations are completed, hindering efficient parallelization of the training process.

In response to these challenges, a novel learning methodology, termed local learning, has emerged \cite{belilovsky2019greedy,mostafa2018deep,bengio2006greedy,nokland2019training,illing2021local,wang2021revisiting}. Contrary to Backpropagation(BP), local learning segments end-to-end backpropagation independently, dividing the network into various local module. 
Local learning rules utilize a gradient-isolated auxiliary network with local objectives to train each layer independently, thereby avoiding the need for backpropagating error signals from the output layer. As a result, local learning can mitigate the update locking problem since each layer updates its parameters independently, facilitating efficient parallelization of the training process. Moreover, unlike BP, local learning does not necessitate the storage of intermediate network states, resulting in significantly lower memory consumption.

However, as pointed out by \cite{bengio2006greedy, belilovsky2019greedy}, local learning might overemphasize local features. While this can enhance local performance, over-learning lower-level local information can trap the network in local optima, thereby compromising the global performance of local learning in comparison to traditional backpropagation.

Subsequent studies \cite{xiong2020loco, wang2021revisiting, siddiqui2023blockwise} have endeavored to tackle this issue. Such as InfoPro \cite{wang2021revisiting} refined the loss function to guarantee that the gradient-isolated network module maintains features beneficial to the overall network during the learning process. However, these methods cannot solve the issue of insufficient interaction between independently optimized layers, resulting in disappointing performance when the network is divided into a large number of independently optimized layers. The performance is particularly unsatisfactory when applied to large-scale networks with numerous independently optimized layers {\cite{deng2009imagenet}}.


\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{sec/20231110-160226.jpg}

   \caption{The HiLo overall architecture. 
   Where (a) is the structure diagram of E2E training, (b) is the structure diagram of other supervised local learning, (c) is the structure diagram of HiLo. We divide the backbone into K blocks in the figure.}
   \label{Figure 1}
\end{figure*}
In this paper, we propose a solution to this problem, which we refer to as Hierarchical Locally Supervised Learning (HiLo). HiLo comprises two forward paths with identical structures but different granularities. The weights of the same module in the different forward paths are shared. Both forward paths adopt a method based on supervised local learning, where the networks in the two forward paths produce different losses through different auxiliary networks. After applying weights, these two losses are summed up to update the weights of the two gradient-isolated network modules simultaneously. The two losses at different granularities can learn different characteristics, thereby compensating for each other's shortcomings. Our overall contributions are as follows:

\begin{itemize}
    \item We have proposed a network structure for the first time in the field of supervised local learning that can truly solve the problem of information interaction between layers.
    \item We have proposed a universal method in the field of supervised local learning, which can be plug-and-play in any supervised local learning methods.
    \item Our proposed HiLo greatly enhances the performance of supervised local learning methods, achieving state-of-the-art results while significantly saving GPU memory compared to E2E method.
\end{itemize}

==> sec/3_method.tex <==
\section{Method}

\subsection{Supervised Local Learning}
In supervised local learning, many previous related studies {\cite{belilovsky2019greedy,mostafa2018deep,bengio2006greedy,nokland2019training}} have enhanced learning capabilities by simply partitioning the network into blocks, and designing an auxiliary network for each block. 
These methods are easy to implement and can greatly save GPU memory. Assuming we have a trainable neural network $Z_{\Theta}: \mathrm{X} \rightarrow \mathrm{Y}$, and we partition this network into K gradient-isolated network modules, where the input sample in the forward propagation process is $x \in \mathrm{X}$, we can write the training process of the network as follows:

\begin{equation}
Z_{\Theta}(x)=f \circ n^k \circ n^{k-1} \circ \cdots \circ n^1(x)
\end{equation}

\noindent where $\circ$ represents the combined function of the neural network, $f(\cdot)$ stands for the final classifier, $n^k(\cdot)$ indicates the operation of the k-th local neural network module, where $1 \leq k \leq K$, and $\Theta=\{\theta^1, \theta^2, \cdots, \theta^k\}$ shows the set of trainable parameters in the neural network.

When we are training the k-th local neural network block $n_{\theta^k}^k$, its training process can be written as:

\begin{equation}
n_{\theta^k}^k(x)=\eta^k \circ \phi^k \circ m^k(x), (1 \leq k \leq K-1)
\end{equation}

\noindent here $\theta^k$ means the trainable parameters in the k-th gradient-isolated network module, $\eta^k(\cdot)$ represents the classification layer in the k-th network module, $\phi^k(\cdot)$ and $m^k(\cdot)$ indicate the functions of the auxiliary network and the main network of the k-th local neural network, respectively.

The optimization objective during the entire training process can then be written as follows:

\begin{equation}
\min _{\Theta, \theta} (\mathcal L\left(Z_{\Theta}(x), y\right)+\sum_{k=1}^{K-1} \mathcal L^k\left(\eta^k\left(\phi^k\left(m^k(x)\right)\right), y\right))
\end{equation}

\subsection{Motivation}
As mentioned above, in the training process of current supervised local learning methods {\cite{illing2021local,wang2021revisiting}}, each gradient-isolated network module updates its parameters through its independent auxiliary network. This means that they are to a certain extent very shortsighted. The reason is that they cannot obtain global error signals {\cite{schultz2000neuronal}}, which causes them to pay too much attention to local error signals. This shortsightedness can impact the overall performance of the model in several ways:
\begin{itemize}
\item {\bfseries Local Optima:} Given that each module is optimizing based on local error signals, it is possible for a module to settle into a local minimum that is good for that module but not good for the overall network performance.

\item {\bfseries Lack of Coordination:} Since each module is not aware of the global error signal, they can't coordinate their learning with other modules. This lack of coordination can lead to inefficiencies and sub-optimal performance {\cite{hawley1995nutritional}}.
\end{itemize}

Based on the aforementioned issues, it is crucial to facilitate information communication between each gradient-isolated network module. If each block could receive feedback from subsequent blocks, it could mitigate this shortsightedness to some extent. To establish a bridge for information communication between modules, we designed a Hierarchical Locally Supervised Learning method for supervised local learning, as shown in Figure \ref{Figure 1}(c). Specifically, we partition the same Encoder in two ways. The left partition enables information sharing between modules, by connecting each block with its immediately adjacent block as a whole for forward propagation. On the right side, it is the same as other supervised local learning methods, where the Encoder is split into single independent blocks for forward propagation. 

In the left-side forward propagation process, each block gets some context from its subsequent block, which might help it learn more global or high-level features. On the other hand, the right-side forward propagation process allows each block to focus on learning local features independently without being influenced by other blocks.By combining these two methods, the model could potentially learn both local features and more global, high-level features more effectively. The local features could help the model to capture fine-grained details in the data, while the global features could help it to understand the broader context or structure of the data. The features they learn complement each other to a certain extent, which helps to further enhance the overall performance of the network.

\subsection{HiLo Design}

We call this training method we designed 'HiLo: Hierarchical Locally Supervised Learning', During the training process, we first duplicate the network's input sample $x$ as $y$, and input them separately into the two different forward channels. During the training process, the parameters of each block in the network are updated by balancing the loss of the two forward channels with a hyperparameter $\alpha$. Specifically, when training the k-th block, the loss of the two forward channels can be obtained as follows:

\begin{equation}
\mathcal{L}_x^k=CrossEntropy(\eta_x^k \circ \phi_x^k \circ res^k \circ res^{k-1}(x), T)
\end{equation}

\begin{equation}
\mathcal{L}_y^k=CrossEntropy(\eta_y^k \circ \phi_y^k \circ res^k(y), T)
\end{equation}



\begin{equation}
\mathcal{L}^k=\left\{
     \begin{aligned}
     & \alpha \times \mathcal{L}_y^k+(1-\alpha) \times \mathcal{L}_x^k, (2\leq k \leq K - 1)\\
     & \alpha \times \mathcal{L}_y^k, k=1
     \end{aligned}
     \right.
\end{equation}

\noindent where $T$ represents the training target of the network, from the above process, we can see that the parameter updates for each pair of split network blocks, $res^k$ and $res^{k-1}$, are achieved through the backpropagation {\cite{rumelhart1985learning}} of $\mathcal{L}^k$.

It is worth noting that the classifiers $\eta_x^k$, $\eta_y^k$ and the auxiliary networks $\phi_x^k$, $\phi_y^k$ in the two forward channels possess different gradients. These differences are purposefully introduced to enable them to concentrate on the distinct characteristics of their respective feature learning. More specifically, they are designed to focus on learning more global features and more local features, respectively. We ultimately amalgamate their losses through the hyperparameter $\alpha$, allowing the network to concurrently acquire both global and local features and thereby achieve optimal performance.


\begin{table*}
  \centering
  \resizebox{0.85\linewidth}{!}{
  \begin{tabular}{@{}lccccc@{}}
    \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{ResNet-32} & \multicolumn{2}{c}{ResNet-110} \\ 
    \cline{3-6}
    & & K=8 (Test Error) & K=16 (Test Error) & K=32 (Test Error) & K=55 (Test Error) \\ \hline
    \multirow{6}{*}{\begin{tabular}{@{}c@{}}CIFAR-10 \\ (BP(ResNet-32)=6.37,\\
    BP(ResNet-110)=5.42)\end{tabular}}  
    & PredSim & 20.62 & 22.71 & 22.08  & 24.74 \\ 
    & \textbf{PredSim*} & \textbf{14.04 ($\downarrow$6.58)} & \textbf{15.92 ($\downarrow$6.79)} & \textbf{16.75 ($\downarrow$5.33)} & \textbf{18.48 ($\downarrow$6.26)} \\ 
    & DGL & 11.63 & 14.08 & 12.51 & 14.45 \\ 
    & \textbf{DGL*} & \textbf{8.37 ($\downarrow$3.26)} & \textbf{9.44 ($\downarrow$4.64)} & \textbf{8.93 ($\downarrow$3.58)} & \textbf{9.56 ($\downarrow$4.89)} \\ 
    & InfoPro & 11.51 & 12.93 & 12.26 & 13.22 \\ 
    & \textbf{InfoPro*} & \textbf{8.24 ($\downarrow$3.27)} & \textbf{9.59 ($\downarrow$3.34)} & \textbf{8.99 ($\downarrow$3.27)} & \textbf{9.35 ($\downarrow$4.27)} \\  \hline
    \multirow{6}{*}{\begin{tabular}{@{}c@{}}STL-10 \\ (BP(ResNet-32)=19.35,\\
    BP(ResNet-110)=19.67)\end{tabular}} 
    & PredSim & 31.97 & 32.90 & 32.05 & 33.27 \\
    & \textbf{PredSim*} & \textbf{28.45 ($\downarrow$3.52)} & \textbf{29.12 ($\downarrow$3.78)} & \textbf{31.04 ($\downarrow$1.01)} & \textbf{31.75 ($\downarrow$1.52)} \\ 
    & DGL & 25.05 & 27.14 & 25.67 & 28.16 \\ 
    & \textbf{DGL*} & \textbf{20.68 ($\downarrow$4.37)} & \textbf{21.93 ($\downarrow$5.21)} & \textbf{21.94 ($\downarrow$3.73)} & \textbf{22.63 ($\downarrow$5.53)} \\ 
    & InfoPro & 27.32 & 29.28 & 28.58 & 29.20 \\ 
    & \textbf{InfoPro*} & \textbf{23.92 ($\downarrow$3.40)} & \textbf{25.54 ($\downarrow$3.74)} & \textbf{24.55 ($\downarrow$4.03)} & \textbf{25.73 ($\downarrow$3.47)} \\ \hline
    \multirow{6}{*}{\begin{tabular}{@{}c@{}}SVHN \\ (BP(ResNet-32)=2.99,\\
    BP(ResNet-110)=2.92)\end{tabular}} 
    & PredSim & 6.91 & 8.08 & 9.12 & 10.47 \\
    & \textbf{PredSim*} & \textbf{5.71 ($\downarrow$1.20)} & \textbf{6.74 ($\downarrow$1.34)} & \textbf{7.01 ($\downarrow$2.11)} & \textbf{8.35 ($\downarrow$2.12)} \\ 
    & DGL & 4.83 & 5.05 & 5.12 & 5.36 \\ 
    & \textbf{DGL*} & \textbf{3.31 ($\downarrow$1.52)} & \textbf{3.74 ($\downarrow$1.31)} & \textbf{3.36 ($\downarrow$1.76)} & \textbf{3.68 ($\downarrow$1.68)} \\ 
    & InfoPro & 5.61 & 5.97 & 5.89 & 6.11 \\ 
    & \textbf{InfoPro*} & \textbf{4.37($\downarrow$1.24)} & \textbf{4.77($\downarrow$1.20)} & \textbf{4.33 ($\downarrow$1.56)} & \textbf{4.92 ($\downarrow$1.19)} \\  \hline
  \end{tabular}}

  \caption{ Comparison of supervised local learning methods and BP on image classification datasets.
The averaged test accuracies and standard deviations are reported from three independent trials.}
  \label{Table 1}
  
\end{table*}


